LLM-Powered Proactive Data Systems

With the power of LLMs, we now have the ability to query data that was previously impossible to query, including text, images, and video. However, despite this enormous potential, most present-day data systems that leverage LLMs are reactive, reflecting our community's desire to map LLMs to known abstractions. Most data systems treat LLMs as an opaque black box that operates on user inputs and data as is, optimizing them much like any other approximate, expensive UDFs, in conjunction with other relational operators. Such data systems do as they are told, but fail to understand and leverage what the LLM is being asked to do (i.e. the underlying operations, which may be error-prone), the data the LLM is operating on (e.g., long, complex documents), or what the user really needs. They don't take advantage of the characteristics of the operations and/or the data at hand, or ensure correctness of results when there are imprecisions and ambiguities. We argue that data systems instead need to be proactive: they need to be given more agency -- armed with the power of LLMs -- to understand and rework the user inputs and the data and to make decisions on how the operations and the data should be represented and processed. By allowing the data system to parse, rewrite, and decompose user inputs and data, or to interact with the user in ways that go beyond the standard single-shot query-result paradigm, the data system is able to address user needs more efficiently and effectively. These new capabilities lead to a rich design space where the data system takes more initiative: they are empowered to perform optimization based on the transformation operations, data characteristics, and user intent. We discuss various successful examples of how this framework has been and can be applied in real-world tasks, and present future directions for this ambitious research agenda.

==> figures/figure1.tex <==
% Define a style for the special labels (for 1, 2, 3)
\begin{tikzpicture}[
    >=Stealth,     % arrow tips
    thick,         % line thickness
    node distance=2.5cm
]

%--- User (person) on the left ---
\node[
  person,
  minimum size=1.25cm,
  label=below:User
] (user) {};

%--- Rectangle in the middle: "1" inside, "operations" below ---
\node[
  draw,
  rectangle,
  minimum width=2.0cm,
  minimum height=1.2cm,
  label=below:operations,
  right=of user
] (box) {\textcircled{1}};

%--- Cylinder (DB) on the right ---
\node[
  draw,
  cylinder,
  shape border rotate=90,
  aspect=1.5,
  minimum height=1.5cm,
  minimum width=1cm,
  label=below:DB,
  right=of box
] (db) {};

%--- Bidirectional arrows with special labels ---
% Arrows between user and box labeled "3"
\draw[->] (user) to[bend left=10] node[above]{\textcircled{3}} (box);
\draw[->] (box)  to[bend left=10]  (user);

% Arrows between box and DB labeled "2"
\draw[->] (box)  to[bend left=10] node[above]{\textcircled{2}} (db);
\draw[->] (db)   to[bend left=10]  (box);

\end{tikzpicture}

==> introbkp.tex <==
\section{Introduction}





Large volumes of real-world data is unstructured, and data systems have long been working towards providing capabilities for the users to store, processes and access unstructured data, through various systems such as data lakes, document stores, semi-structured databases, etc. With the significant improvement of AI models and particularly LLMs in performing natural language tasks, many data systems have incorporated LLMs to perform data processing tasks on unstructured data. Such tasks include automated information extraction from unstructured data, better data integration, other data transformations such as generating summaries and data enrichment, and better search over such datasets. Data system interfaces furthermore allow users to interact with the system through natural language, even if the data itself is structured.

However, many applications of LLMs in such systems consider LLM operations as given, where LLMs perform black-box operations as specified by user input on data monolithic, where, similar to any other UDF, the data system neither understands the data or the task, but performs them as it's told. We call such data systems \textit{reactive}: the database system is given the reactionary role of executing user operations, without understanding the user intent, the specified operation or the data where it should be applied. We believe reactive data systems are inherently flawed, limiting the ability of the system to accurately and efficiently answer user questions. To understand the limitations of reactive database systems, consider the following example. 

\begin{example}\textit{(Police Misconduct)}
     Consider a dataset of police files containing reports about police investigations into an incident. To ensure police accountability, a journalist may be interested in finding cases where the police were accused of misconduct. To accurately satisfy the journalists needs, the system needs to be able to:
     \begin{itemize}
         \item \textit{(Understand the Task)}. The query of ``find me instances of police misconduct'' is difficult to process accurately since misconduct is never directly stated in police records. The system needs to understand and decompose the task, e.g., into ``was there use of force in a police incident'' and ``was the use of force justified''.
         \item \textit{(Understand the Data)}.  The system needs to understand the data to identify what portions can be relevant. There can be repeating patterns that can be exploited, e.g., instances of misconduct may be found in specific sections of documents. Finding relevant portions of the document can be both improve accuracy and reduce cost 
         \item \textit{(Understand the Intent)}. The system needs to adjust to user intent through feedback. Misconduct can have different meanings, and the journalist may be interested in specific types, e.g., racial biases. The system needs to interact with the user and refine data processing to match the intent. 
     \end{itemize}
\end{example}
\if 0
\begin{example}\textit{(Understanding the Task)}
     Consider a dataset of legal contracts
\end{example}

\begin{example}\textit{(Understanding the Data)}
     understanding data
\end{example}

\begin{example}
     \textit{(Understanding Intent)}. On either a structured or unstructured data source stating containing names of people, consider the simple query of a user asking for records of ``Adam Smiht'', where ``Smiht'' is a misspelling of ``Smith''. The system needs to understand user intent (which name they are asking for). This may need to be done with respect to data (e.g., if neither ``Smith'' or `'Smiht'' exist, the answer is the same for both queries). The system cannot ensure correctness by always correcting what it perceives as typos, there may be deviations from common name spelling that are not typos. 
\end{example}
\fi

We argue that the database systems need to be proactive. They need to be given agency to understand user intent, data operations, and the dataset, and to make decisions on how to processes the user-provided operations. In the police misconduct example, this means breaking down the task, finding patterns in the data and interacting with user to find their intent. Such operations are now possible by using LLMs as tools to understand users, data and data transformations better, both on structured data or unstructured data. We believe the three axes of understanding (1) user intent, (2) data operations and (3) the data 
itself are the key to the data systems' ability to accurately and efficiently processes structure and unstructured data. 

\sep{will come back to this paragraph after the rest of the paper}The design space of proactive database systems is huge since our problem formulations are open-ended. For example, a task may be decomposed in many different ways and simply using an LLM as an agent to make all decision leads to inaccurate results. Taking inspiration from our prior work, we discuss various solutions on how proactive data systems can make progress in the three abovementioned axes. For each axis, we discuss various knobs at our disposal, such as performing decompositions and rewrites to improve accuracy when performing a task, finding structure in unstrcutred data to better understand the data and answer queries on it, and by adjusting data and query representations based on user feedback to better align the system with user intents.  We discuss future directions along each axis to build better proactive database systems. 





\if 0


\newpage

Use-cases:
- police records: llm needs to organize data, needs to interact with user to decide how, what are relevant features, differ some decisions to user (e.g., check decide how to check if two police officers with the same name are the same person). 
- NL queries: intent discovery, when there needs to be multi hop interactions with user. Bring up TableQA, what if a user specifies a wrong predicate, returning information not strictly asked by the user but may be what the user is asking for


\textit{A post-relational data model is a data model based on the principle that the relational data model is no longer sufficient or necessary to represent the real-world.}

\begin{itemize}
    \item Lots of text/video data, people want to process/query text/videos
    \item Even with relational data people want to query with NL. Database might be getting queried without clear/specific intent. Dataset search
    \item Overall, both data and/or query can be fuzzy and lack structure
    \item Police records example
\end{itemize}

\begin{itemize}
    \item  Relational DBMSs are not well-suited to handle the above
    \item They rely on mathematical abstractions to provide a declarative interface defined based on the data
    \item This leaves the burden of translation of real-world information needs outside of the dbms
    \begin{itemize}
        \item E.g., NL to SQL, or structured information extraction before interacting with the database
    \end{itemize}
    \item To be more accurate and efficient dmbs should be responsible for answering such queries, without necessarily relying on relational data model
\end{itemize}


\begin{itemize}
    \item We believe the above observation necessitates a rethinking of what abstractions and interfaces a dbms needs to provide, and how that affects the internals of a dmbs.
    \item Criticism of the relational model that it does not capture real-world semantics existed in the 70s when it was proposed. Methods such as ER diagrams and entity relationship models were proposed to bridge such a gap. In recent years, the lack of real-world semantics has become even more apparent as AI is used to perform the human-level tasks. e.g., NL2SQL methods have to rely on meta-data (data catalogs and column descriptions) and external knowledge to formulate queries correctly, and poor integratiions with a dmbs can lead to suboptimal results.  
    \item  However, many recent work accept the relational model, but replace specific tasks that is designated to humans within this model, e.g., NL2SQL or automated schema extraction. 
    \item Instead, we consider relational model as a specific point in data management design space, and question its design choices, given that assumptions that existed when it was proposed  (i.e., the ability/intelligence of a machiine) are no longer true
\end{itemize}
    



\begin{itemize}
\item Specifically we argue that dmbs should natively support both unstructured and structured queries on unstructured and structured data, leading to a decoupling of interface provided by the system vs internal data representations and definitions. 
\item We discuss how this change in the abstraction in a dbms can change the interface and internal design choices, in terms of internal data/query representation and planing
\item Overall, prior visions depict the LLM as a tool that can help us translate new data into the relational model, but we believe scope of dmbs should be expanded in the presence of LLMs as opposed to fit new data/query sources into existing relational framework
\end{itemize}

\fi

==> old/design_space.tex <==
\section{The Data Management System Design Space}
\subsection{Rethinking abstactions and internals of dbms}
\begin{itemize}
    \item We consider (1) what query/data interface systems support and (2) the internal data and query representation
    \begin{itemize}
    \item The above two are the same in relational database systems, which provide a declarative intereface on the relational data, where SQL instructions are dependendent on the (logical) structure of the data, as internally represented
    \end{itemize}
    \item In the interface, database should allow for both unstructured and structured interface, where data/queries can be unstructured (e.g., RAG on text), structured (SQL on relational), or somewhere in between (e.g., zendb)
    \item Internally, a dbms can decide to translate the user input/store and represent data in a structured or unstructured way
    \begin{itemize}
        \item Structure can be used to improve accuracy/efficiency, but does not necessarily exists
    \end{itemize}
    
\end{itemize}

\subsection{Why does it matter}
\begin{itemize}
    \item Relational databases store data as a materialized structured projection of the real-world, and provide a query language to query the data based on this pre-defined structure. 
    \begin{itemize}
        \item This projection is based on a pre-defined workload for the application designed by the DBA, This is good if
        \item  There is a fixed and pre-defined workload, from which a needed structure can be deduced
        \begin{itemize}
            \item The structure repeats in the data (i.e., tables have multiple rows)
        \end{itemize}
        \item The structure is known by users of the system so that they can query it
        \begin{itemize}
            \item queries need data based on the same logical structure as defined for the data
        \end{itemize}
        
    \end{itemize}
\end{itemize}
\begin{itemize}
\item However, information needs from a real-world phenomenon is not necessarily fixed or predictable, and may not follow and obvious predefined structure. Even if structure exists, it might not be known to the user. Examples:
    \item Police records
    \item Legal documents
    \begin{itemize}
        \item Information not adhering to the predefined structure
    \end{itemize}
    \item Civic meetings agenda
    \begin{itemize}
        \item Information with a mix of structure and unstructured data (e.g., some structure repeats, but some doesn’t.) Can be fixed entities but each entity has different attributes, or each query can be asking for different attributes. 
    \end{itemize}
    \item some dataset search example
    \item AI allows querying such data, so requires rethinking what are good abstractions and how database internals should change. There are bad alternatives, discussed below. 
\end{itemize}

\subsection{Bad solutions}
\begin{itemize}
\item “LLM calls as UDFs” 
\begin{itemize}
    \item Bad abstraction, stops from performing a lot of optimizations 
\end{itemize}
\item “DMBS is relational, the rest of the data/query must just be translated (outside of the dmbs) to relational“
\begin{itemize}
    \item Can be suboptimal because sometimes unstructured representation is more accurate/efficient
    \item Can be suboptimal because of poor integration of translation from unstructured to structued
\end{itemize}
\end{itemize}

==> old/system.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{db.pdf}
    \caption{Database Design}
    \label{fig:design}
\end{figure}

\section{Design of Post-Relational Data Management Systems}
Figure~\ref{fig:design} shows an overview of how we envision a post-relational data management system to look like. 

The system consists of three main workflows (1) database design, (2)  data ingestion and (3) query answering. The design workflow is in charge of deciding the logical and physical design of the database based on user-provided data and query definitions, as well as (potential) database redesign based on newly observed queries and data records. The data ingestion workflow is in charge of parsing data records to map them to the logical and physical design. The query answering workflow is in charge of answering user queries. We first discuss the user interface of the system, and then discuss in more details the internals of the database for each of the three workflows mentioned. We end the section by discussing some algorithmic components common to the different workflows within the system.

%The first two are instigated by user interaction (e.g., database setup, new record insertion, asking new query), the third can happen in the background but can take user interactions into account (e.g., database agent can decide to reorganize database after observing a number of queries to be better optimized for a workload). 


\subsection{Interface}
The user interacts with the system to either define what data and queries are to be handled database, or to query or modify the data in the database. We call the former the Data and Query Definition Interface, and the latter two comprise the Data Manipulation Interface. These interfaces support natural language inputs from the user and may provide natural language outputs. Thus, an important aspect of the two interfaces is having the human in the loop to ensure correctness of the results. We first describe the two interfaces, and then provide more details on the human in the loop nature of the interfaces. 

%Data ingestion part of the system is a collection of components in the system that take (1) data definition and (2) data records as input and create (1) metadata describing the data and how its stored and (2) physical blocks where data is stored.

%In relational dbms this layer is straight forward. Data definition is done using DDL in SQL and the DML layer provides instruction to support modification and query of new data records as defined by DDL instructions. Simple implementation, just requires parsing, and data layout design decides how to store data. Different storage choices are made to improve efficiency, but no discussion of accuracy since everything is mathematically well-defined. Extensions beyond relatinoal models increases importance of this layer, no well-defined mapping of how things should logically be stored



\subsubsection{Data and Query Definition Interface}
Data and Query Definition Interface allows users to define how to insert or query their data. The interface itself can be in different levels of structure, from supporting only structured operations such as DDL in SQL in one end to just providing a natural language interface where users can provide a description of the data to be inserted and queries to be performed on the system. 

The interface has two important features. First, because the interface support natural language the system may need to ask follow up questions to resolve ambiguities, understand intent or allow user to validate the outputs. As such, the interface can be interactive, as further discussed in Sec.~\ref{sec:hil}.  Second, the interface allows decoupled Data and Query Definitions. That is, logical data representation does not need to correspond to the logical query representation. This allows the user to define SQL schema on unstructured data, or natural language schema on structured data. Allowing different query and data definitions is important and gives the database system the agency to decide how the data should be mapped to the query. That is, by having a decoupled query and data interface, the system allows all data transformation, extraction, loading, and integration choices to be differed from the data management system. We provide a two examples below. 


\textbf{SQL Queries on Unstructured Data}. The system may define a schema so that queries are performed in SQL, while the input to the system may be unstructured data, as done in ZenDB \cite{lin2024towards} and ELEET \cite{urban2024efficient}. This defers to the system to decide how to map the unstructured data to the query schema. Although performing ETL upfront is possible, both approaches advocate against such a methodology and perform retrieval and extraction on the fly. This shows how decoupling data and query definition allows the system to perform the mapping between the two themselves, providing a richer optimization space that can be exploited by the database system.  

\textbf{Definitions for Unstructured Query and Data}. When either query or data are unstructured, providing additional information about the data or query are important. For example, when doing natural language query on rational data additional meta-data containing description of tables, columns and extra information that can be used to query is important to allow for query answering (for example, BIRD \cite{li2024can} benchmark for NL2SQL provides meta-data about columns and tables). Even when data and queries are unstructured users can provide instructions on how they should be processed. In our police records example, users can provide hints for the system to cluster different police cases. Such definitions allow users to provide additional domain knowledge and information about future queries that help the system decide how to organize the data. 


Overall the data and query definition interface allows users to navigate between a fully relational database and a RAG system. As different application utilize different levels of structure in either query or data, we envision a database system that supports all such specifications. 

%The interface allows users to defined what data will be inserted into the system and what queries will be performed. Users can define query interface and data insertion interface that are different (i.e., do not adhere to the same schema). Overall, the users can define \textit{Structured Query and Data}: This is how data is traditionally defined in relational dbms. Users to define tables, data types, constraints, etc. \textit{Structured Query on Unstructured Data}: Users can define a structured query interface while allowing unstructured data to be inserted. ZenDB, ELEET. \textit{Unstructured Query on structured datar}: Users can define schema to insert data, but allow users to perform unstructured query NL2SQL, TableQA, dataset search. \textit{Unstructured Query on Unstructured Data}: Retrieal/RAG applications. \textit{Semi structured data/queries}: There is usually some amount of structure. Even in the classical unstructured text retrieval, a corpus is divided into a set of documents, rarely it's just a blob of text with nothing known about it. One can do things like DocETL which uses some structure (e.g., applying the same operation across documents), or define additional operations (e.g., some predefined LLM call user can do). 



%The DDI interface itself can be structured or unstructured, just provide data description. Can defin base

%DDI allows users to define how they interact with DBMS and how data can be inserted and accessed. The users can define interfaces that are



\subsubsection{Data Manipulation Interface}
After data and query definition, the user can interact with the system to insert/update/delete data (data ingestion) and to perform query queries. The interfaces follow their respective definitions where data ingestion and/or query interface can be require structured inputes or not. In addition to (or instead of) performing the operations requested by the user and returning the result, the interface may need to ask follow-up questions to do intent discovery or disambiguation. The interface may also need to provide tools for the user to validate the operations performed by the database. The system may raise errors if it cannot semantically parse and perform the operation. We further discuss the interactive interface in Sec.~\ref{sec:hil}

%. (1) when users perform queries or insertions, the interface provides tools for users to verify the operations, for example by showing provenance. And (2) the systems may engage in interactive querying if the system decide the operation cannot be performed just based on user input. This may require additional follow ups to the user to do intent discovery, to disambiguate the query or the data. 


\subsubsection{Human in the Loop}\label{sec:hil}
Because the interface allows natural language input, understanding what the user and/or data mean may require additional interactions with the user. This may require intent discovery to understand user queries and disambiguation of data. Moreover, the user needs to be able to verify the operations performed by the user. Thus, the system needs to provide tools for the user to verify operations. This can be in various forms, for example, asking users for labels, and measuring accuracy to ensure it satisfy some user defined requirement. It can also be in terms of showing provenance to the user, or other explainability artifacts to show what the system has done. An example is showing the SQL query to user if the system perform NL2SQL. 


\subsection{Database Design workflow}
The database design workflow takes instructions provided by the user in the data and query definition interface and designs the logical and physical representation of the data. It physically creates and stores the relevant meta-data that will later be used to decide how and where to insert new data records, as well as how to map queries to the observed data points.

In relational dbms this workflow is straightforward. Data definition is done using DDL in SQL, and the system only needs to parse DDL instructions and create the relevant meta-data (i.e., schema) to be stored physically. Design choices on how the data is stored are for efficiency purposes only (e.g., columnar, materialize views, index, etc.). %, where the main question if physical data representation, given that logical representation is given/known. 
%and the DML layer provides instruction to support modification and query of new data records as defined by DDL instructions. Simple implementation, just requires parsing, and data layout design decides how to store data. Different storage choices are made to improve efficiency, but no discussion of accuracy since everything is mathematically well-defined. 
On the other hand, extensions beyond the relational model increase the importance of this workflow since the user may not have provided a mathematical definition of the logical data structure. As such, the system needs to decide how to logically and physically store the data. Internally, this workflow consists of three components: (1) parsing user input, (2) logical representation design and (3) physical representation design. 

\subsubsection{Parsing}
This component parses user instructions, decides if additional user feedback is needed (e.g., in cases of ambiguity), and raises errors if it cannot parse user instructions (errors can be both from inability to parse semantically or syntactically.). 

%Syntax check, check for potential ambiguity, ask follow up question (similar to other parsing components mentioned in more details in the other two workflows)

\subsubsection{Logical Representation Design}
The system then decides what the logical representation of the data should be. In cases when the user defines the logical representation, the system just relies on user provided definitions. However, the system can be responsible for designing a logical representation of the data,

\textbf{User-defined Representations}
If the user specifies the logical representation of the data, then the system relies on the provided definition. This can be data schema in a relational setting, but there are many other possibilities. For example, the user can simply specify that data is a collection of documents, each broken into smaller text chunks of a certain size, to store the data in a vector database. Moreover, unstructured data can be defined as an additional column in an already existing schema to combine structured and unstructured data. 

\textbf{Automated Representation Design}
Alternatively, when given unstructured data, the system can decide how to logically represent the data. The system can decide to create a schema based on the data and create an information extraction pipeline to transform unstructured data to a structured format, or can decide to keep data as a collection of unstructured text chunks and store them in a vector database. Such a choice can be made based on the amount of structure available in the data and the required task.

For example, in cases of semi-structured data, EVAPORATE \cite{arora2023language} extracts information and inserts them into a structured table. On the other hand, Semantic Hierarchical Trees in \cite{lin2024towards} create a logical view of the information in a document by identifying different sections in the document and building a tree hierarchy that represent information in the text. Moreover, the data representation can be self-improving, and specialized for tasks. For instance, NUDGE \cite{zeighami2024nudge} optimizes data representations for the specific query workload in hand. 

Overall, users during data and query definition, users can provide a task (or set of tasks they want to do) and description of the data and the system needs to break down the task and decide how data should be stored based on the task. This can require deciding what information is relevant, and how it should be extracted and stored it. Besides the system may also need to decide how different records are related (e.g., orginze different files in police records), and decide to build different collections of data records used for downstream tasks.


\subsubsection{Physical Storage Design}
The system also needs to decide what needs to be physically stored and how to stored. If the system is adhering to user-defined representation, then physical storage may be well-understood, e.g., in case of relational or vector databases. However, when system automatically design the logical data representation, it further needs to decide what needs to be stored and how. Moreover,  need to decide what level of user feedback and workload to store to allow the database to improve over time based on queries and user interactions. Overall, physically, the system will store meta-data, data and any query workload and user feedback information needed. 
%Physical data storage based on logical data representation. Need to decide how to physically store the logical representation as meta-data and the corresponding data. Also 

\textbf{Meta-Data}. Meta-data includes information about the logical data representation, and allows the system to use the logical data representation to physically find relevant data. In relational dbms, this includes schema information and where the corresponding data is stored. In post-relational dbms, the meta-data can include additional information such as extracted structure, summaries of records, user-provided description, virtual views and mappings between logical data representation and possible locations to find the data (For example, as done in ZenDB\cite{lin2024towards}). 


\textbf{Data}. Based on logical data representation, the system may decide to store multiple physical data representations. Each data representation may be useful for different workloads, or can provide varying levels of accuracy when answering queries. For example, system may extract some of the fields, create data embeddings, summaries, or may simply store text as is.

\textbf{Query workload and user feedback}. System also decide how to store the query workload and user provided feedback. A simple approach is to just store all queries and any feedback the user provides. This may get too costly, and the system can decide what needs to be kept based on the data definition and existing levels of ambiguity (e.g., store more feedback on ambiguous records, where more impact is expected).

\subsection{Data Ingestion workflow}
Data ingestion takes data records as input and stores it in physical blocks in the database and performs any meta-data changes needed. The parsing component may decide to ask follow-up questions from the user, or raise errors if it cannot parse the data. The storage components uses the meta-data to figure out where and how the data needs to be stored, and performs necessary operations to translate the input into the required format. The operations here can include a combination of the traditional Extract, Transform and Load operations when data is unstructured.



\subsubsection{Parsing}
This component takes data input from user, and attempts to map it to the logical representation designed for the data. In addition to syntactic errors, there can be semantic errors, where data may not adhere to existing or predefined semantics. Semantic assertions such as in SPADE\cite{shankar2024spade} can be used to ensure data quality. 

The system performs both syntactic parsing (e.g., for cases where there is any expected pre-defined structure) or semantic parsing to understand the logical representation of the data and how it fits in within the existing database. In our police records examples, this means finding the correct file where a new record belongs, or potentially raising an error if it cannot be assigned to any existing file. Other parsing strategies are possible, for instance ZenDB\cite{lin2024towards} extracts structure from a templatized document and checks if the template matches templates in other existing documents.  
%\textbf{Syntactic Parsing}. If there is any amount of structure there can be syntax checks to match the structure

%\textbf{Semantic Parsing}. Parse the data to make sure it matches data definition. This can be semantic operations, e.g., if there are collection of different police records, this step can semantically understand where the record belongs, or raise an error if the record does not belong to any of the predefined categories. It can also figure out if there is an error, e.g., if a police record doesn't have a date.

%If the system needs to do some sort of semantic mapping, then the system can ask the user for verification, or provide some sort of provenance for why the type of mapping happened for users to check. The system should decide when/how often the validation should happen, what records to validate to minimize human involvement while maximizing accuracy. 

%Can do zendb's template matching to see if the data matches existing templates

%The system can also check for ambiguity and raise errors if it the level of ambiguity passes some amount of certainty

\subsubsection{Storage}
If the data record is semantically valid and understandable by the system, then the system needs to store it in the database based on the designed physical storage scheme. This may require extracting certain information and/or performing data transformations. This stage performs such transformations and writes the data to the physical storage, with any additional meta-data and user feedback generated. This process is reminiscent of existing ELT workflows and can be done using methods such as DocETL~\cite{shankar2024docetl}. However, in contrast with ETL pipelines, this process need not be a one-off ETL of all existing data. Instead, the system can decide if any ETL is needed what operations to perform and can perform various Extract, Transform or Load operations throughout the lifecycle of the database. 

\subsection{Query Processing}
At query time, the database uses the stored meta-data and data to answer queries. The system may ask follow-up questions and interact with the user in multiple rounds after searching the database. Thus, in general, query answering can be a multi-step process. Intrnally, to process the query, the system performs (1) parsing to understand the query, (2) planning to decide how to answer the query and (3) execution which performs certain planned steps on the data. The three steps are not necessarily done once and sequentially and may be interleaved with each other. 

\subsubsection{Parsing}
Similar to data ingestion, parsing is an important component that goes beyond syntactic parsing. This step requires mapping the query to a logical representation that can be used to find the relevant data. This step can require semantic operations to map the query to the logical data representation. Similar to all other user interactions in the system, the system may ask follow-up questions to resolve ambiguities. Moreover, the system may need to use the data and perform intent discovery to understand what information the user is looking for. 


\subsubsection{Planning and Execution}
Given a (possibly partial) logical representation of the query, the system needs to decide what operations to perform. The system may not be generating a complete a complete query plan, since the query may require asking follow-up from the user. This step outputs specific LLM call or mathematical operations that can be performed on the database and/or user query. The execution engine then executes the plan. 

To maximize accuracy of the system and minize the cost, the system can try to optimize the plan and its execution.  This can be done using rewrite methods, such as in DocETL~\cite{shankar2024docetl}, cascade, caching, compression, filtering, etc. We give an overview of various algorithmic components that can be used for optimization throughout the database in Sec.~\ref{sec:alg_opt}. 




%\subsubsection{Verification and Provenance}
%User should be able to verify operations. e.g., show SQL to user if we end up doing NL2SQL or other forms of provenance. Can be other forms of provenance, e.g., show text where data was extracted in ZenDB. 

\subsection{Algorithmic Componenets}\label{sec:alg_opt}
Having a good system requires in general to have methods to maximize accuracy while minimizing both amount of compute and human involvement. Below is general discussion of various tools in our disposal 

\textbf{Utilizing Hidden Structure}. Important tool when operating on unstructured data is that there is often hidden structure. Extracting and using the structure often helps improve accuracy and/or cost. It helps decomposing and rewriting tasks into simpler logical unit and decomposing data into logical units, which both help with reducing cost (i.e., to avoid looking at entire dataset) and improving accuracy, since model is better at doing simpler tasks. DocETL, ZenDB

\textbf{Reducing amount of data processed}. We can often filter and/or compress data to reduce the amount of information llms needs to look at. This can be done by extracting relevant fields, filtering using embeddings, creating summaries or doing other prompt compression techniques (e.g., stuff by Trummer). 

\textbf{Re-using processed data}. We can use caching (prompt caching, prefix matching stuff) or creating materialized views to avoid reprocessing the data


\textbf{Model-based improvements}. We can fine-tune models to get better for the data. We can use cheaper models 

\textbf{Human Cost Optimizations} Deciding what should be labeled to minimize interactions with user, probably cite some crowdsourcing work

\textbf{LLM Agents}. Various parts of the system requires performing open-ended tasks, give that inputs are not necessarily structured. e.g., how to breakdown query, how to structure the data, figuring out if can the query be answered given the data, or if the logical structure of data is good based on user feedback.  Performing such actions can be done by LLM agents, that are good at making such open-ended operations, perhaps by additional guidance (e.g., DocETL). Agents don't necessarily have to be LLM agents, nor are a new thing (RL agents were used for query optimization XXX or database tuning XXXX), but LLM agents are good/new because they can perform open-ended tasks and operate in an unstructured space.




==> subsections/system_task_processing-old.tex <==
%!TEX root=../main.tex


\section{Proactive Operation Understanding and Reformulation}
In reactive data systems, the onus
is on the user to author queries involving
the ``right'' LLM-powered operators,
with the system then determining how to execute
these in conjunction with other relational operators.
However, even in cases where users
are able to specify clear, unambiguous operations,
the granularity at which they specify them may
not be optimal for execution.
Fundamentally, this stems from a lack
of understanding of what LLMs can do well
versus what they can't---something most users
are not aware of.
In this section, we discuss various 
approaches to 
operation reformulation 
that can improve accuracy 
while maintaining or reducing computational costs.

\topic{Decomposition into simpler LLM operations}
In Example~\ref{ex:police}, we described
how sometimes journalists want to extract
dozens of fields from a given document
(e.g., police officer names, descriptions
of misconduct, locations, use of firearms, among others).
The journalist may specify the entire list of fields
along with instructions within a prompt.
However, executing this as is in a single LLM call
may lead to poor accuracies
as LLMs often struggle to identify multiple concepts simultaneously~\cite{shankar2024docetl}.
A proactive system can decompose such an operation
into separate focused ones that
each extract one type of information, improving
accuracy.
An LLM can be asked rewrite a prompt that
says ``extract fields f$_1$, ..., f$_n$ from the following ...''
into ``extract field f$_i$ from the following ...''.
In prior work, we have identified
several new decomposition-based rewrite rules~\cite{shankar2024docetl}
that can lead to higher accuracies,
when coupled with LLMs being used to instantiate
the rewrites themselves.
Recent work on Text-2-SQL also leverages 
similar ideas~\cite{pourreza2024chase}: 
rather than attempting translation 
in ``one-shot'' (i.e., single LLM call), 
which often fails due to schema mismatches 
or poorly-named schemas~\cite{luoma2025snails}, 
it is beneficial to 
parse the operation into smaller units, e.g.,
given ``find all employees who joined before 2020'', 
first identify the core concepts: employee records 
and hire dates,
and treat each separately.

\topic{Leverating non-LLM components}
In certain cases, operations
that are assigned to an LLM may be better done
through other means, e.g., through SQL.
For example, finding the average settlement amount 
for misconduct cases can be decomposed 
into an LLM operation to 
identify relevant cases and their settlement amounts, 
followed by a SQL aggregation to compute the average.
We have employed similar techniques where
we separate operations that require real-world reasoning (suited for LLMs) from mathematical computations (better handled by traditional database engines or calculators) in
our work on ZenDB~\cite{lin2024towards}.
Determining how to do this automatically
may be challenging, but we may be able to use 
reasoning models for this purpose. 

\topic{Leveraging LLMs to assess benefits}
One question that naturally emerges when considering
decomposing operations into smaller units
is how to assess the benefits of such decompositions.
While it is a-priori hard to tell whether
a decomposition will help, we can run
both the non-decomposed and decomposed
variants on a sample. 
LLMs are much better at evaluating outputs
than generating them, so LLMs can be used
to tell which version performs better.
For example, 
one can employ a ``generate-fix \& rewrite-verify'' pattern: generate an initial operation formulation, 
verify its correctness (e.g., through automated checks or LLM verification), and if verification fails, attempt alternative formulations~\cite{chung2025long}. 
This pattern, which we also use in DocETL~\cite{shankar2024docetl}, allows a system to systematically explore the space of possible task formulations until finding one that passes verification, effectively optimizing for accuracy through trial and refinement.
However, doing evaluation in a cost-effective manner remains
a challenge. 


\topic{Calibrating LLM outputs}
Independent of which decomposition is used,
when LLMs are independently being applied
to a set of items (documents, tuples),
the outputs can often be
inconsistent and non-calibrated.
For example, if we ask LLMs to rate
the severity of every incident
in our document collection,
it often gives all of them the same score,
or worse, gives them scores that
are only losely correlated with the severity.
To remedy this lack of consistency,
we can take various actions.
We can leverage the LLMs themselves to pick 
representative examples that indicate
the full range of the categories of interest, provided
as few-shot examples.
Or they can rework the prompt to describe in more detail
the criteria used for evaluation---to ensure consistency.
Finally, they can also
restrict the space of possible outputs
(e.g., when LLMs are asked to extract state information
from a collection of US addresses, they may extract CA in some
cases and California in others).
While this doesn't change the semantic meaning of the operation, it can significantly improve LLM accuracy by providing better context and guidance, as has
also been explored in work on prompt optimization~\cite{khattab2023dspy}.


\topic{Deferring to cheaper LLMs for the ``easy bits''}
One concern with decomposition is that
it may increase the cost of the overall pipeline,
since one LLM call per document may now become
multiple. 
One way to defray the cost is to couple decomposition
with cost optimization:
for the simpler newly decomposed operations,
we can alternatively use cheaper and smaller
models to handle them, and only use the more expensive model 
for the most complicated operations.
For example, when we're trying to extract many fields
from a police record document, we can use a cheaper
model for extraction of locations and dates, while using
a more expensive model for harder tasks such as
determining the type of misconduct incident.
While the idea of cheaper proxy models isn't new~\cite{},
here, since the space of decompositions is infinite,
and for each decomposition (or sequences thereof), 
we could use different
models and different confidence thresholds, each with 
different cost-accuracy tradeoffs, the problem
becomes a lot more compliacated.
Additionally, unlike previous settings which focused primarily on tasks with well-defined accuracy metrics, we now must provide guarantees for open-ended generative operations---where quality is harder to quantify.

 
\topic{Expensive predicate ordering, but with synthesized predicates}
For operations that involve subselecting documents
based on certain criteria (all expressed
together in one prompt), we can leverage existing
related work on expensive predicate ordering~\cite{};
however, in our context, we can introduce an arbitrary
number of new dependent predicates (that are potentially easier
to check and therefore cheaper).
For example, instead of using an expensive model
to examine each police record document to extract
medical impacts to the victims, if any,
we can consider cheaper filters
that are easier to check, for example, 
if the document contains any medical information at all.
This check could potentially be done by a cheaper
model and rule out a substantial fraction of the documents.
Similarly, when decomposing a complex filter like ``find 
incidents involving both use of force and drug use'' into two 
filters, one for ``use of force'' and one for ``drug use,'' the 
system can evaluate the more selective filter first to minimize expensive LLM calls.








\topic{Leveraging reasoning for reformulate}
As described above, a proactive data system
must reformulate (e.g., decompose or rework) operations to better execute them. However, finding good reformulations is difficult. Current approaches to discovering task reformulations are quite naive. Systems like DocETL simply prompt LLMs to suggest rewrites, either taking the first suggestion or selecting from multiple candidates. One option is to use a powerful ``reasoning'' model like OpenAI's o1 model to rewrite the task, but this still fundamentally relies on one-shot prompting, and is unaware of how the rewrite will actually perform on the data. We need approaches that can learn what characteristics of the data make tasks challenging, what types of LLM errors occur in different contexts, and use this knowledge to guide task reformulation---perhaps even in an agentic fashion.


\topic{Coalescing into more complex operations}

















\agp{old content follows}
\subsection{Semantic Operation Rewrites}

One strategy to improve operation accuracy is to rewrite it based on our {\em semantic} understanding of what it does. There are several strategies to perform semantic rewrites:

\textbf{Decomposition into Simpler Operations}. Consider Example~\ref{ex:police} where journalists extract various information like locations and police officers from misconduct records. While a user might write this as a single well-specified operation (``find locations and police officers mentioned in the case''), executing this prompt directly may lead to poor accuracy since LLMs often struggle to identify multiple concepts simultaneously~\cite{shankar2024docetl}. By semantically understanding the operation, a proactive system can decompose it into separate focused operations that each extract one type of information, improving both accuracy---and even enable parallelization, improving latency.

\textbf{Hybrid Operation Decomposition}. Semantic understanding also enables decomposing operations into LLM and non-LLM components. Systems like ZenDB~\cite{lin2024towards} demonstrate the value of separating operations that require real-world reasoning (suited for LLMs) from mathematical computations (better handled by traditional database engines). For example, finding the average settlement amount for misconduct cases can be decomposed into an LLM operation to identify relevant cases and their settlement amounts, followed by a SQL aggregation to compute the average. 

\textbf{Semantic Parsing for Operation Translation}. Semantic understanding can also improve accuracy when translating natural language to SQL queries~\cite{pourreza2024chase}. Rather than attempting translation in a ``one-shot'' manner (i.e., single LLM call), which often fails due to schema mismatches or poorly-named schemas~\cite{luoma2025snails}, a proactive system could first parse the operation into semantic components. For instance, given ``find all employees who joined before 2020'', the system identifies the core concepts: it needs employee records and hire dates. Only then does it map these semantic concepts to actual database objects.

Semantic rewrites can be combined with database optimization techniques to reduce costs. For example, when decomposing a complex filter like ``find incidents involving both use of force and drug use'' into two filters, one for ``use of force'' and one for ``drug use,'' the system can apply traditional query optimization principles like filter reordering. By understanding that these are independent predicates, it can evaluate the more selective filter first to minimize expensive LLM calls. \shreya{Of course, there might be correlation between the predicates}

\subsection{Non-Semantic Rewrites}

Beyond semantic understanding, systems can improve operation accuracy through systematic reformulation and verification:

\textbf{Generate-Fix-Verify Pattern}. Some NL-to-SQL approaches employ a ``generate-fix \& rewrite-verify'' pattern: they generate an initial operation formulation, verify its correctness (e.g., through automated checks or LLM verification), and if verification fails, they attempt alternative formulations~\cite{chung2025long}. This pattern, also seen in DocETL~\cite{shankar2024docetl}, allows a system to systematically explore the space of possible task formulations until finding one that passes verification, effectively optimizing for accuracy through trial and refinement.

\textbf{Prompt Engineering}. Operations can be reformulated by enriching them with carefully selected examples, failure cases, or more expressive descriptions. While this doesn't change the semantic meaning of the operation, it can significantly improve LLM accuracy by providing better context and guidance~\cite{khattab2023dspy}.

\shreya{Stopped here for now}

\subsection{Challenges and Future Directions}

\textbf{Systematically exploring Task Reformulations}. A proactive database system reformulates tasks so that it can better execute them. However, finding good reformulations is difficult. Current approaches to discovering task reformulations are quite naive. Systems like DocETL simply prompt LLMs to suggest rewrites, either taking the first suggestion or selecting from multiple candidates. One option is to use a powerful ``reasoning'' model like OpenAI's o1 model to rewrite the task, but this still fundamentally relies on one-shot prompting, and is unaware of how the rewrite will actually perform on the data. We need approaches that can learn what characteristics of the data make tasks challenging, what types of LLM errors occur in different contexts, and use this knowledge to guide task reformulation---perhaps even in an agentic fashion.

%Moreover, we need better ways to predict LLM behavior on different types of tasks---both to avoid costly reformulations that won't improve accuracy, and to identify when verification steps needed to . %Second, these agents need cost models that can reason about the tradeoffs between different LLM models and traditional database operations in a unified way. Current approaches either ignore costs entirely or treat LLMs as black-box UDFs with fixed costs, neither of which captures the complexity of modern LLM pipelines.


\textbf{Cost-Aware Reformulations}. Moreover, oprations involving LLM operations can be prohibitively expensive, especially when processing large datasets. We can turn to AQP. By understanding which tasks (or components of tasks) can be approximated using cheaper LLMs or simpler operations, we can reduce cost without significantly impacting result quality. For instance, we might use smaller models for initial filtering steps, or perform operations on a sample of the data when high precision isn't required. While these strategies are well-known, modern LLM-based systems pose new challenges. For one, instead of simply choosing between a cheap proxy model and an expensive oracle, systems must now reason about hundreds of potential models and multi-step pipelines, each with different cost-accuracy tradeoffs. Additionally, unlike traditional AQP which focused primarily on tasks with well-defined accuracy metrics, we now must provide guarantees for open-ended generative operations---where quality is harder to quantify.

%Data systems increasingly support tasks specified in various ways, ranging from pure SQL queries, to natural language questions, to SQL queries augmented with AI-based functions or predicates for natural language reasoning (e.g., {\tt SELECT * FROM documents WHERE llm\_classify(text, "this document contains police misconduct") = TRUE}). However, the way users specify these tasks may not be optimal for execution, whether due to limitations of the underlying data model, capabilities of the execution engine, or ambiguity in the specification itself. 

% \subsubsection{Breaking Down Complex Operations}
% A proactive database system can decompose complex operations, that is, break them down into series of steps, in order to improve accuracy and lower costs. 
 
% \textbf{Decomposition into Simpler Tasks}. Consider our Example~\ref{ex:police} where the journalists are interested in extracting various information, such as locations, police officers involved, etc., from police misconduct records. A user might write this as a single operation, executing the prompt ``find locations and police officers mentioned in the case'' against all police incident records. While simple to write, executing this prompt on the documents as-is may lead to poor accuracy, if the LLM struggles to identify multiple concepts simultaneously~\cite{shankar2024docetl}. A proactive system could rewrite this into separate focused operations that each extract one type of clause, thereby improving both accuracy and even latency by parallelizing the task.

% \textbf{Decomposition with Tool Use}. This decomposition principle extends beyond just splitting LLM operations. Systems like ZenDB~\cite{lin2024towards} demonstrate the value of separating operations that require real-world ``reasoning'' (suited for LLMs) from mathematical computations (better handled by traditional database engines). For example, finding the average settlement amount for misconduct cases might involve an LLM to identify relevant cases, followed by a SQL aggregation function to correctly compute the average. \shreya{TODO: discuss tool usage}

% \textbf{Optimizing Cost}. Breaking down tasks also enable cost optimization. In our Example~\ref{ex:police}, consider a journalist looking for incidents involving both use of force and drug use. Writing an LLM-based pipeline to execute the prompt ``Does this incident involve use of force and drug use'' against all documents, can lead to unnecessary expensive solutions if one of the conditions, e.g., ``use of force'', is highly selective. An LLM might be able to quickly filter out many documents if it first decomposes the prompt into ``Does this incident involve use of force`` and  ``Does this incident involve drug use''. That is, by reordering these filters and minimizing cost by pushing selective filters down in the query plan~\cite{liu2024declarative}. Beyond enabling such filter reordering, decomposing tasks can unlock other optimization opportunities—from parallelizing independent LLM operations, to caching intermediate results, to selecting different LLMs for different subtasks based on their complexity.

% \if 0
% if one of the filters is very selective. For example, if very few incidents involve use of force, find relevant legal documents: {\tt SELECT * FROM documents WHERE llm\_filter(text, "discusses patent infringement AND involves pharmaceutical companies")}. Even if the ``patent infringement'' condition is highly selective and could quickly filter out many documents, the LLM evaluates both conditions together for every document, if it is treated like a black box. Ideally, a proactive system would rewrite this into two separate filters:

% \begin{verbatim}
% SELECT * FROM documents 
% WHERE llm_filter(text, "discusses patent infringement")
% AND llm_filter(text, "involves pharmaceutical companies") 
% \end{verbatim}

% Then,  we can reorder these filters---minimizing cost by pushing selective filters down in the query plan~\cite{liu2024declarative}. 
% \fi



% \subsubsection{Semantic Parsing}
% A proactive database system can semantically parse a user input to be able to map it better to the data. Consider performing natural language queries on a relational database. Modern NL-to-SQL systems rely heavily on LLMs to generate SQL queries directly from the user's query and database information. However, enterprise settings often involve hundreds of tables with complex schemas, making it impossible to include complete schema information in LLM prompts \shreya{TODO: cite}. Even when schema information fits in the context window, these systems often fail when schema details don't match the LLM's expectations---even subtle variations in column names (e.g., ``rec\_id'' versus ``record\_id'') can cause incorrect SQL generation \shreya{TODO: cite arun kumar paper}. 

% Rather than trying to generate SQL directly, a proactive system first understands the {\em meaning} of the query. For example, given ``find all employees who joined before 2020'', the system might first decompose this into its {\em conceptual} components: it needs an entity representing people employed by the company, and a temporal attribute representing when they started. Only then does it map these semantic concepts to actual database objects---finding that {\tt employees} maps to the {\tt hr\_personnel} table and {\tt joined} maps to {\tt start\_date}. Such a semantic parsing of the task into a logical representation can help bridge the gap between how users express their information needs, and how data is structured in the database. It can also allow the system to ensure the operations performed are semantically correct. The system can through semantic errors if it cannot semantically understand user inputs. 


% \subsubsection{Task Rewrites}
% %Semantic rewrites can be particularly powerful when combined with verification. 
% A proactive database system can rewrite the task so that it can be better executed by the system. The task statement can be enriched with examples, failure possibilities, more expressive descriptions, etc. to improve accuracy.

% Such rewrites are often coupled with a verification mechanism. In many cases, we can verify the correctness of an LLM's output, for example through automated checks (e.g., testing if a generated SQL statement is valid), comparing results against known examples, or using another LLM as a verifier. This ability to verify opens up new optimization strategies. Systems like CHASE-SQL and various NL2SQL approaches \shreya{TODO: cite} employ a``generate-fix-verify'' pattern: they generate an initial task formulation, verify its correctness, and if verification fails, they attempt alternative formulations. For instance, if an LLM generates incorrect SQL due to misunderstanding column names, verification would catch this error, and the system could try reformulating the query. This pattern, also seen in DocETL~\cite{shankar2024docetl}, allows a system to systematically explore the space of possible task formulations until finding one that passes verification, effectively optimizing for accuracy through trial and refinement.


% \subsubsection{Challenges and Future Directions}

% \textbf{Systematically exploring Task Reformulations}. A proactive database system reformulates tasks so that it can better execute them. However, finding good reformulations is difficult. Current approaches to discovering task reformulations are quite naive. Systems like DocETL simply prompt LLMs to suggest rewrites, either taking the first suggestion or selecting from multiple candidates. One option is to use a powerful ``reasoning'' model like OpenAI's o1 model to rewrite the task, but this still fundamentally relies on one-shot prompting, and is unaware of how the rewrite will actually perform on the data. We need approaches that can learn what characteristics of the data make tasks challenging, what types of LLM errors occur in different contexts, and use this knowledge to guide task reformulation---perhaps even in an agentic fashion.

% %Moreover, we need better ways to predict LLM behavior on different types of tasks---both to avoid costly reformulations that won't improve accuracy, and to identify when verification steps needed to . %Second, these agents need cost models that can reason about the tradeoffs between different LLM models and traditional database operations in a unified way. Current approaches either ignore costs entirely or treat LLMs as black-box UDFs with fixed costs, neither of which captures the complexity of modern LLM pipelines.


% \textbf{Cost-Aware Reformulations}. Moreover, oprations involving LLM operations can be prohibitively expensive, especially when processing large datasets. We can turn to AQP. By understanding which tasks (or components of tasks) can be approximated using cheaper LLMs or simpler operations, we can reduce cost without significantly impacting result quality. For instance, we might use smaller models for initial filtering steps, or perform operations on a sample of the data when high precision isn't required. While these strategies are well-known, modern LLM-based systems pose new challenges. For one, instead of simply choosing between a cheap proxy model and an expensive oracle, systems must now reason about hundreds of potential models and multi-step pipelines, each with different cost-accuracy tradeoffs. Additionally, unlike traditional AQP which focused primarily on tasks with well-defined accuracy metrics, we now must provide guarantees for open-ended generative operations---where quality is harder to quantify.



% \shreya{Outline:
% \begin{itemize}
%     \item Users specify tasks in many ways; in SQL, in natural language, or some hybrid combination.
%     \item However these tasks are specified, it might be suboptimal given the data model (or lack of data model), or given the capabilities of the execution engine. For example, imagine the LLM is the execution engine; scanning a legal document to extract many types of clauses. We know LLMs are bad at doing many things in one go, so we may rewrite this query to be k independent queries, each of which extract a small number of clauses. Moreover, tasks can also be ambiguously specified---especially if natural language---and a rewrite of the task can bring at least some specificity to the query, thereby improving the quality of the result (give an example here)
%     \item There are several ``types'' of query rewrites, or ways to think about query rewrites. One is along logically decomposing a complex task into a sequence of simpler tasks. Another is to separate ``reasoning'' from mathematical operations, that databases and data processing engines will do well (e.g., ZenDB), or tasks well-executed by other tools (e.g., getting the weather). Another is to approximate definitions when the query is ambiguous (todo: figure out how to say this better)
%     \item What's key here is to do this {\em agentically}, that is, semantically understand the task, rather than rely on user-specified decompositions. In a simple example, imagine the user has written a pipeline with 2 filter operations. A system like Palimpzest will reorder the filters cost-optimally. However imagine they wrote the pipeline with one filter operation, where the operation was described by a prompt that effectively squishes both the predicates together, joined by the word ``and.'' We should ``agentically'' break this prompt into its 2 different operations, perhaps with an LLM, and then apply our cost optimization---rather than leave the operation as-is.
%     \item NL to SQL: it seems like being ``aware'' of the data model is very difficult, especially in enterprise data, where there are too many tables to fit in a prompt, and it's not even clear what the tables are. cite also Arun Kumar's work of LLMs getting confused by column names, like ``rec\_id'' and ``record id'', LLMs do not correctly generate the SQL if the column name is the former
%     \item Generate-fix-verify pattern in CHASE-SQL and NL2SQL; if we have a verifier (can even be an LLM), then we can put the system to keep trying alternative task formulations in a loop. DocETL also leverages this
%     \item Future directions: how to effectively search over different task decompositions---DocETL's strategy of ``just ask the LLM for different decompositions'' is a start, but how can we be smarter about it, find these decompositions in a data-driven way or based on what the LLM gets wrong? , approximate query processing---figure out what tasks (or part of tasks) are easy to approximate with cheaper LLMs, cost and accuracy aware optimization, developing agents for task rewriting (that can consider the appropriate context) with the generate-fix-verify or TAG paradigm
% \end{itemize}
% }

% \textbf{Query rewrites} DocETL things that go here, rewrites to approximate user intent, rewrites to enjoy better system performance, rewrites to improve accuracy (given limitations of LLMs)

% \textbf{Task Decomposition} DocETL things that go here, also ZenDB-style (and LLM UDFs) hybrid LLM + SQL queries

% \textbf{Future Directions}
